Building AI Agents for Autonomous Clouds: Challenges and Design Principles

The rapid growth in the use of Large Language Models (LLMs) and AI Agents as part of software development and deployment is revolutionizing the information technology landscape. While code generation receives significant attention, a higher-impact application lies in using AI agents for operational resilience of cloud services, which currently require significant human effort and domain knowledge. There is a growing interest in AI for IT Operations (AIOps) which aims to automate complex operational tasks, like fault localization and root cause analysis, thereby reducing human intervention and customer impact. However, achieving the vision of autonomous and self-healing clouds through AIOps is hampered by the lack of standardized frameworks for building, evaluating, and improving AIOps agents. This vision paper lays the groundwork for such a framework by first framing the requirements and then discussing design decisions that satisfy them. We also propose AIOpsLab, a prototype implementation leveraging agent-cloud-interface that orchestrates an application, injects real-time faults using chaos engineering, and interfaces with an agent to localize and resolve the faults. We report promising results and lay the groundwork to build a modular and robust framework for building, evaluating, and improving agents for autonomous clouds.

==> motivation.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[scale=0.4]{Figures/lifecycle.png}
  \caption{Incident lifecycle}
  \label{fig:lifecycle}
  \vspace{-1em}
\end{figure}

\section{Background: Challenges of Operating Cloud Services}
\label{sec:example}
\pb{0.5pgs}
%\own{Pedro/Minghua take an initial look}
% 
\ys{fold in with relatred work first para}

\ms{thinking-out-loud: not sure this section adds much (particularly wrt to motivation). IMO, describing in intro an example of an "advanced" AIOps soln making mistakes + what users deploying them in production need--compare tools, explainability--motivates better.}\ys{agreed. we need to go beyond the surface.}

% \ys{may be useful to walk thru an example based on first hand knowledge. Case studies, experiences of fault detection, triaging, localization, and mitigation. Our internal motivation for such a tool. Severity metrics, human cost, biz impact. Need for Reliability, efficiency.}
%\ys{Gagan, who would be best place to write this part? Adds a unique first-hand perspective and establishes our authority on the subject (given it is double blind review).}


We offer a brief overview of the lifecycle of a fault incident detection and mitigation with the use of AIOps tools to help ground these requirements and design choices.
CompanyX, the organization behind this study, operates thousands of application deployments within massive, globally distributed cloud data centers, catering to millions of users. Incidents are a common occurrence, and clear protocols have been established by various operational teams for managing and escalating these incidents within the Incident Management System (IcM). The incident management process (\cref{fig:lifecycle}) for handling cloud service incidents encompasses four key stages: 

\ys{could we add details of \textit{how} they perform each of these steps? Whats tools they use? E.g., logs, traces, documented steps. Challenges they face?}

\begin{itemize}[leftmargin=*]
\item \textbf{Detection}: Incidents are detected automatically by monitoring systems or manually by engineers and reported to the IcM system.
\item \textbf{Triage}: On-Call Engineers (OCEs) are notified to begin investigation and assign the incident to the most relevant team.
\item \textbf{Mitigation}: The assigned team diagnoses the issue and takes action to mitigate it, such as rebooting service or roll over changes.
\item \textbf{Resolution}: After mitigation, a thorough analysis is conducted to identify the root cause, fully resolve the incident, and update postmortem in the IcM system.
\end{itemize}

Mitigating incidents promptly is crucial, as extended Time To Mitigate (TTM) can result in reduced service availability and significant financial losses. The complexity and scale of systems often make manual investigation and mitigation by engineers expensive. 

\ys{could we include some statistics to highlight the scale and impact? faults seen per day, number of sev 1 and sev 2 faults? time to resolution? person-hours consumed and escalation (VP gets called?)? business impact.}
